Addressing Topic Granularity and Hallucination in Large Language Models for Topic Modelling

Large language models (LLMs) with their strong zero-shot topic extraction capabilities offer an alternative to probabilistic topic modelling and closed-set topic classification approaches. As zero-shot topic extractors, LLMs are expected to understand human instructions to generate relevant and non-hallucinated topics based on the given documents. However, LLM-based topic modelling approaches often face difficulties in generating topics with adherence to granularity as specified in human instructions, often resulting in many near-duplicate topics. Furthermore, methods for addressing hallucinated topics generated by LLMs have not yet been investigated. In this paper, we focus on addressing the issues of topic granularity and hallucinations for better LLM-based topic modelling. To this end, we introduce a novel approach that leverages Direct Preference Optimisation (DPO) to fine-tune open-source LLMs, such as Mistral-7B. Our approach does not rely on traditional human annotation to rank preferred answers but employs a reconstruction pipeline to modify raw topics generated by LLMs, thus enabling a fast and efficient training and inference framework. Comparative experiments show that our fine-tuning approach not only significantly improves the LLM's capability to produce more coherent, relevant, and precise topics, but also reduces the number of hallucinated topics.

==> ideas.tex <==
1. we find this issue based on our experiments

2. previous work uses extra steps

3. our work without extra steps
we are the first

4. DPO add equations for DPO loss

5. add a figure to show the full pipeline of our work


==> notes.tex <==
add additional results via open review after the submission due

1. improve the introduction based on our experiments

2. update the full draft

3. polish the tables and figures to make it clear and informative

4.



5. improve Fig 1.
-- add rules and dynamic seeds topics in fig.1

6. re-run the third experiments

7. presentation of the approaches for each points / eva


presentation Xingyi's suggestions
discussion of my plans to improve the paper
paper structures
paper draft ---> discussion and conclusion
add more methods
add more prompt tuning approach
add special tokens

to do list:
1. paper structure

--- %\section{Problem Definition or Background}
% Describe the problem and background here

%section{method}
%subsection{zero shot}
%subsubsection{Prompting Strategy}
%describe results and pinpoint the results section
%subsection{DPO fine-turning}
% Start with DPO background 
% acc rej instruct
%subsubsection{Reconstruction pipeline}

% \section{Experiments}
% dataset
% splits
% base model 
% baseline models
% evaluation metrics

% \section{results}
% discussion
% sum

***vera website to promote our work 
check out Olesya's draft (the SemEval one) in vera.ai.com
revision 


(1) Google Docs with images with main contributions,
topics
*to Johann 

(2) ack for the papers, 

right acknowledgments,

check it with Kalina and Xingyi
* make sure to use the correct ACK in the camera-ready paper; some grants have been done;

content 
spatio temporal paper


2. one more dataset


